Reachability-based Trajectory Safeguard (RTS): A Safe and Fast Reinforcement Learning Safety Layer for Continuous Control

Reinforcement Learning (RL) algorithms have achieved remarkable performance in decision making and control tasks due to their ability to reason about long-term, cumulative reward using trial and error. However, during RL training, applying this trial-and-error approach to real-world robots operating in safety critical environment may lead to collisions. To address this challenge, this paper proposes a Reachability-based Trajectory Safeguard (RTS), which leverages reachability analysis to ensure safety during training and operation. Given a known (but uncertain) model of a robot, RTS precomputes a Forward Reachable Set of the robot tracking a continuum of parameterized trajectories. At runtime, the RL agent selects from this continuum in a receding-horizon way to control the robot; the FRS is used to identify if the agent's choice is safe or not, and to adjust unsafe choices. The efficacy of this method is illustrated on three nonlinear robot models, including a 12-D quadrotor drone, in simulation and in comparison with state-of-the-art safe motion planning methods.

==> Sections/Deprecated.tex <==
\subsection{How does RTSA get integrated into training}
\begin{outline}
\1 In online operation, our RTSA module lies in between the network and LLC. On the one hand, it acts as a safety layer for the parameters RL output, ensuring that when RL selects an unsafe set of parameters, it is replaced by the safety layer to a set of parameters that don't collide with the obstacle. 
\1 On the other hand, it acts as a reference trajectory generator, generating parameterized continuous and achievable trajectories for the low level controller(LLC) and dynamics. 
\1 Essentially, the green box in Figure \ref{fig:Framework} is a new environment that is safe by construction. 
\1 We perform Model-Free reinforcement learning on that safe environment, therefore ensuring zero collision during learning and operation.
\end{outline}


\begin{outline}
\1 RTS takes inspiration from RTD, using parameterized reference trajectory to generate the FRS of the Robot to ensure safety.
\1 This method can be applied to nonlinear systems given a Low Level Controller
\1 In \textbf{Offline} operation: A high fidelity FRS is computed by sampling a parameterizable planning model(PRS) and bouding the tracking error(ERS) for all samples

\1 In \textbf{Online} operation: The set of parameters selected by the network undergoes safety-check in parameter space. if that set of parameters does not pass safety check, a alternative set of safe parameters are found and used to generate reference trajectory for the LLC.


\end{outline}








\begin{outline}
%\2 Using CORA, the trajectory producing model can be 
\1 Obtaining the Tracking Error Function (ERS)\label{sec:ers}
\2 We call the position error in each dimensions of the workspace the tracking error. Given some assumptions, we bound the tracking error g(t,k,xi) for each set in parameter space K. 
\2 We approximate g by sampling reference trajectories in parameter space, and recording the maximum error between reference and (simulated) real system for each t, k interval and xi interval.
\shrey{we can reference ch. 6 of my dissertation for how to do this sampling conservatively}
\2 In past work, we add the maximum footprint to the tracking error of the center of mass, to obtain the over-approximating FRS. 

\2 In this work, to further reduce conservatism, we combine footprint and tracking error by computing tracking error of the all vertices of the robot with respect to the reference trajectory at sampled time instants. Then, we find the convex hull of the tracking error of all vertices for an set of target parameters
\3 an example of finding ERS using such a method is shown in Figure \ref{fig:ERS}

\2 Using Minkowski sum, we combine the tracking error and trajectory producing model, obtaining a slice-able collection of \textbf{zonotopes} representation of the full FRS of the robot over a time horizon.
\end{outline}





\begin{outline}
% \1 Obstacle representation
% \2 We assume obstacles are static and compact. Therefore, the convex hull of obstacles of arbitrary shape can be represented as zonotope objects in workspace
% \2 As the robot moves, each obstacle enters the sensor horizon of the robot and is converted to a zonotope representation. 
% \1 Slicing 

% \2 Before obstacle check, we \textbf{slice} the sequence of zonotopes by the initial condition of the robot.\simon{(How to deal with when initial condition is in the future??), dont worry about it}
% \shrey{typically we use the high-fidelity model to predict where the robot will end up at time $t\plan$}

% \1 Parameter Space Collision Check
% \2 With FRS saved as a collection of zonotopes and obstacles already in zonotope representation, checking two zonotope intersection is equivalent of using Lemma 8 in the ARMTD paper: Each obstalces are converted halfspace in paraemter space, and checking multiple obstacle is finding the same as finding $\mathbf{max}(Ak-b) >$ 0 for each obstacle
% \2 Iterate over the collection of zonotopes in the time series, we will obtain a linear function that can be quickly evaluated at each parameters to check collision status with each obstacle. 

\1 Parameter Safety Check and Adjustment
\2 We evaluate the function obtained in previous step on the network parameter output. If that combination of parameters does not work, we find the closest set of parameters that works by sampling the parameter space and evaluating sample distance to original parameter.
\2 If it turns out the all other sampled parameters still intersect with the obstacle, we execute the fail-safe plan from the previous verified safe plan
\3 a example of how such a method works online for cars is shown in Figure.\ref{fig:OnlineOps}
\end{outline}

==> Sections/ERSJustificationApp.tex <==
\section{Justifying ERS Conservatism}\label{subsec:justify_ers_conservatism}

We now justify our adversarial sampling strategy for computing the ERS.
In particular, we sample the \textit{corners} of each $K\idxj\times X\hiz\idxh$ to ensure that our ERS representation is conservative as in \eqref{eq:ers_conservatism}.
In short, as one would expect, tracking error is maximized by sampling the largest possible commanded \textit{changes} in the robot's velocity.
When a planning model's velocity is monotonic in $k\ini$ and/or $k\desi$ (which the models we consider are), this implies that one should choose samples of $k$ with the largest possible magnitude.

As a reminder, we require conservatism because, if we \textit{overestimate} the robot's reachable set, then we can ensure the robot is safe by ensuring that its reachable set does not intersect obstacles.

Note that it is reasonable to satisfy \eqref{eq:ers_conservatism} in practice, as validated empirically in both simulation and on hardware for a variety of robot morphologies \cite{kousik2018bridging,kousik2019safe,kousik2020_pcba,holmes2020reachable,shreyas_dissertation,vaskov2019not,vaskov2019towards}.
Moreover, if one is unsure if \eqref{eq:ers_conservatism} is satisfied, one can simply use larger $Z\err\idxerr$.

\subsection{Setup and Assumptions}
We proceed by considering a double-integrator linear system representing the robot's actuators.
We assume that the robot's tracking error is proportional to its actuators' tracking error with respect to a desired acceleration profile.
We also assume that all states in $X\hi$ that are not linear/angular position are the robot's linear/angular velocity; in other words, maximizing acceleration error leads to maximizing position error.

\subsection{Sampling Initial Conditions}
We sample the corners of $X\hiz\idxh$ because tracking error is maximized when initial speed is maximized:
\begin{prop}\label{prop:tracking_error_max_at_max_k_init}
(\cite[Proposition 7.1]{shreyas_dissertation})
Consider a high-fidelity model with states $p$ and $\dot{p} \in \R$, and $\ddot{p} = u \in \R$.
Let $p\plan(\cdot,k): T \to \R$ be a smooth plan.
Suppose that
\begin{align}
    u = \gmp\cdot(p - p\plan) + \gmd\cdot(\dot{p} - \dot{p}\plan) + \ddot{p}\plan,
\end{align}
where $\gmp,\gmd \in \R$ are control gains and $\ddot{p}\plan$ is a feedforward term.
Suppose that $p(0,k) = p\plan(0,k) = 0$ and $\dot{p}(0,k) \in [\dot{p}\submin,\dot{p}\submax]$.
Then the tracking error magnitude $|p(t,k) - p\plan(t,k)|$ achieves a maximum over $t \in T$ and over all $\dot{p}(0,k)$ when $\dot{p}(0,k) \in \{\dot{p}\submin,\dot{p}\submax\}$.
\end{prop}
\noindent Recall that we require $k\ini = f\ini(x\hiz)$, so this proposition justifies sampling the corners of both $K\ini\idxj$ and $X\hiz\idxh$.

\subsection{Sampling Trajectory Parameters}
We sample the corners of $K\des\idxj$ because tracking error is maximized when commanded velocity is maximized:

\begin{prop}\label{prop:tracking_error_max_at_max_k_des}
Consider the model from Proposition \ref{prop:tracking_error_max_at_max_k_init}, and suppose $u$ has no feedforward term:
\begin{align}\label{eq:prop_k_desi_controller}
    u = \gmp\cdot(p - p\plan) + \gmd\cdot(\dot{p} - \dot{p}\plan).
\end{align}
Suppose $p(0) = p\plan(0,k)$.
Suppose $k = (k\ini,k\desi)$ with $k\ini$ fixed such that $\dot{p}(0,k) = \dot{p}\plan(0,k)$.
Consider a planning model $p\plan: T\times K \to \R$ for which, for all $t \in T$, $\ddot{p}\plan(t,k) = k\desi \in [k\submin,k\submax] \subset \R$ (that is, $K\desi$ is also 1-D).
Then the tracking error magnitude $|p(t) - p\plan(t)|$ is maximized when $k\desi \in \{k\submin,k\submax\}$.
\end{prop}
\begin{proof}
Consider the tracking error system
\begin{align}
    z(t,k) &= \begin{bmatrix}
            z_1(t,k) \\ z_2(t,k)
        \end{bmatrix} =
        \begin{bmatrix}
            p(t) - p\plan(t,k) \\ \dot{p}(t) - \dot{p}\plan(t,k)
        \end{bmatrix}.
\end{align}
Recalling that $\dot{k} = 0$ for any plan, we have
\begin{align}
    \dot{z}(t,k) &= \underset{A}{\underbrace{\begin{bmatrix}
            0 & 1 \\ \gmp & \gmd
        \end{bmatrix}}}z(t,k) +
        \begin{bmatrix}
            0 \\ \ddot{p}\plan(t,k)
        \end{bmatrix},\label{eq:prop_k_desi_proof_first_order_system}
\end{align}
for any fixed $k \in K$.
We can solve for $z$ to find
\begin{align}
    z(t,k) &= e^{At}z(0,k) + \int_0^t e^{A(t-s)}\begin{bmatrix}
            0 \\ \ddot{p}\plan(s,k)
        \end{bmatrix}ds\label{eq:prop_k_desi_proof_generic_soln}\\
        &= 0 + \left(\int_0^t e^{A(t-s)}ds\right)\begin{bmatrix}
            0 \\ k\desi
        \end{bmatrix}\\
        &= -A\inv(e^{At} - I_{2\times 2})\begin{bmatrix}
            0 \\ k\desi
        \end{bmatrix},\label{eq:prop_k_desi_proof_particular_soln}
\end{align}
where $I_{2\times 2}$ is an identity matrix.
Notice that
\begin{align}
    A\inv = \begin{bmatrix}
            -\gmd/\gmp & 1/\gmp \\ 1 & 0
        \end{bmatrix},
\end{align}
and we can choose $\gmp$ and $\gmd$ such that
\begin{align}
    e^{At} = \begin{bmatrix}
            a_1(t) & a_2(t) \\ a_3(t) & a_4(t)
        \end{bmatrix}
\end{align}
with $a_2(t)$ and $a_4(t) \neq 0$.
Then, by expanding \eqref{eq:prop_k_desi_proof_particular_soln}, we have
\begin{align}
    z_1(t,k) = \frac{1 - \gmd a_2(t) + a_4(t)}{\gmp} k\desi,
\end{align}
completing the proof.
\end{proof}
\noindent Note that the planning model in this proposition does not obey the requirement that $\dot{p}\plan(t\final,k) = 0$.
We chose this simplification for the sake of illustrating the main idea: the tracking error is proportional to $k\desi$, as one would expect.

Note, one can derive a similar result for a planning model with $\ddot{p}\plan(t,k) \propto (k\desi - k\ini)t^2$ (as is the case for the three robots we consider in this paper) by applying integration by parts to \eqref{eq:prop_k_desi_proof_generic_soln}.
More generally, this result holds (again by applying integration by parts) if $\ddot{p}\plan(t,k) = f_1(k)f_2(t)$ where $f_1$ is a linear combination of elements of $k$ and $f_2$ is a polynomial in $t$.

Furthermore, input saturation does not affect the result of Proposition \ref{prop:tracking_error_max_at_max_k_des}.
Notice that we assume the control input is drawn from $U = \R$, but $U$ is compact for the high-fidelity model.
First, notice that if we include the feedforward term $\ddot{p}\plan$ in $u$ from \eqref{eq:prop_k_desi_controller}, then the tracking error is $0$ for all time without input saturation.
But, if the input is saturated, this is equivalent to a constant control input being applied in the solution to \eqref{eq:prop_k_desi_proof_first_order_system}, meaning that $\ddot{p}$ is a constant as in the proof.
Therefore, as we would expect, one can maximize tracking error by choosing $k\des$ to maximize input saturation (i.e., command the largest possible acceleration).

\subsubsection*{Takeaway}
From the above analysis, it is reasonable to assume that, if we compute the ERS zonotopes as in Sec. \ref{subsubsec:compute_ers_via_sampling}, then they enclose the worst-case tracking error as required in \eqref{eq:ers_conservatism}.

==> Sections/Methods/Enforcing_safety_reach_old.tex <==
\section{Offline Reachability Analysis}\label{sec:offline_reachability}

% \begin{outline}
% \1 overview
%     \2 leverage reachable sets to ensure safety
%     \2 reachable sets allow us to plan with the simplified model while incorporating tracking error
%     \2 offline, we compute a Planning Reachable Set (PRS) of the planning model, and an Error Reachable Set (ERS) of tracking error
%         \3 the PRS lets us identify which of the continuum of possible plans are unsafe in each planning iteration
%         \3 the ERS lets us incorporate tracking error into planning, by adding tracking error to the PRS, which leverages the zonotope Minkowski sum
%     \2 to enforce safety during training and testing, we combine the PRS and ERS into an FRS of the robot's points reachable in workspace when tracking parameterized trajectories; the FRS lets us identify which plans are safe for the RL agent to choose
% \end{outline}

\Ram{I think this entire section will probably need to be removed in the final version and we will just need to point at a reference and say we can compute reach sets..}

This section describes how to compute the Forward Reachable Set by splitting it into a planning reachable set(PRS), which is an over-approximation of the planning model, and an error reachable set(ERS), which is an over-approximation of the forward occupancy map with respect to the planning model. 
In the previous section, we described how to directly compute the plan, add \Ram{is add the right word?} the tracking error, and compute the forward occupancy map of the robot, to ensure its safety with \eqref{eq:safety_def}.
However, doing such a computation online is too slow for real-time operation. 
Furthermore, when needing an alternative plan \Ram{awk}, we have to recompute another forward occupancy map from scratch.

To accelerate this process, we use a combination of offline reachability analysis and online safety verification.
A natural \Ram{what does natural mean? Empty word} way to do such a computation would be to iterate through all plans, generate a Forward Reachable Set(FRS) representing the $\forwardoccupancy(x\hi)$ for each plan, and use these saved FRS online to check for obstacle intersections.
However, such a computation would be intractable due to the continuous parameter space we obtain trajectories from \Ram{this sentence is not written in proper english}.\simon{as well as the continuous high-fidelity initial condition space we obtain initial condition from. remove this for concise?}

As an alternative, we split the FRS to a planning model and a sampling based forward occupancy error map (FOError) \Ram{sampling seems like the wrong word here.}. 
We employ a zonotope representation for both, compute their upper bound, and call them the planning reachable set and error reachable set \Ram{again this is not english}.
By recombining them online, we obtain a overapproximation of the FRS, which we can quickly reference and refine based on the plan and initial condition to ensure safety. 
% In another word, offline, we compute zonotope reachable sets.
% Online (i.e., during training and operation), we use these sets to formulate safety constraints on the trajectory parameters (i.e., plans) in each planning iteration.


This section describes how to compute a Planning Reachable Set (PRS) containing the parameterized trajectories of the planning model.
Second, it describes how to construct an Error Reachable Set (ERS) containing the forward occupancy error of the robot with respect to the planning model.
The next section describes how to combine the PRS and ERS online to construct a Forward Reachable Set (FRS) of the robot tracking the planning model trajectories, and how to use the FRS to identify unsafe plans.

\subsection{Planning Reachable Set}\label{subsec:PRS}

% One can think of the PRS as a function $\PRS: T\times K \to \pow{P\times K}$ for which $(p\plan(t,k),k) \in \PRS(t,k)$, meaning that $\PRS$ is conservative.
We compute the PRS as a set of zonotopes using an open-source toolbox called CORA \cite{althoff2015cora}.
To proceed, we first define zonotopes, explain what data are needed to compute the PRS, and how to compute the PRS as a set of zonotopes.
\subsubsection{Zonotopes}
A zonotope is a set
\begin{align}\label{eq:zono_defn}
    \zono{c,G} = \left\{y \in \R^n\ |\ y = c + G\beta,\ \beta \in [-1,1]^m\right\},
\end{align}
where $c \in \R^n$ is the zonotope's \defemph{center}, $G \subset \R^{n\times m}$ is called a \defemph{generator matrix}, and $\beta$ is called the \defemph{coefficient vector}.
Notice that every point in $\zono{c,G}$ is a linear combination of $c$ with the columns of $G$, which we call the \defemph{generators} of the zonotope.
% Another way to think of this is that a zonotope is an affine transformation of the unit hypercube $[-1,1]^m$.
Also note that a point $c \in \R^n$ is a zonotope with no generators, $\zono{c,[\ ]}$.

\subsubsection{Setup to Compute the PRS}
We provide the toolbox \cite{althoff2015cora} with three inputs to compute the PRS.
First, we provide the planning model as in Definition \ref{def:plan} in the form
\begin{align}
    \dot{z}(t) = \begin{bmatrix}
        \dot{p}\plan(t,k) \\
        0_{\Kdim\times 1}
    \end{bmatrix},
\end{align}
where $z = (p\plan, k)$ is a parameter-augmented state vector.
Second, we provide an initial condition set as a zonotope.
Recall that all plans begin from $0$.
The initial zonotope is
\begin{align}
    Z\plan\idxz &= \zono{c\idxz,G\idxz}\ \subset P\times K,\ \regtext{with} \\
    c\idxz &= (0_{\plandim\times 1},\Kcenter) \in \R^m\ \regtext{and} \\
    G\idxz &= \diag{0_{\plandim\times 1},\Kdelta} \in \R^{m\times m},
\end{align}
where $m = \plandim + \Kdim $.
Third, we partition $T$ into $n_T \in \N$ intervals.
Let $\Delta_T = \frac{t\final}{n_T}$, $T\idx{1} = [0,\Delta_T]$, and $T\idxi = \big((i-1)\cdot\Delta_T, i\cdot\Delta_T\big]$.
Then
\begin{align}
    T = \union_{i=1}^{n_T} T\idxi.
\end{align}

\subsubsection{The Planning Reachable Set}
We use \cite{althoff2015cora} to compute the PRS as a set of zonotopes,
\begin{align}\label{eq:prs}
    \PRS = \left\{Z\plan\idxi = \zono{c\plan\idxi,G\plan\idxi}\ |\ i \in \N_{n_T}\right\}.
\end{align}
One can show using \shrey{cite the theorems} that, if $t \in T\idxi$ and $k \in K$, then
\begin{align} 
    (p\plan(t,k),k) \in Z\plan\idxi.
\end{align}
That is, the PRS contains all possible plans and associated parameters.
\simon{prs needs split too, but introducing the partition here seems early for high fid initial $X\hi$ though, so opt for talking about partition in B}
% \begin{outline}
% \1 offline
%     \2 PRS
%         \3 We make use of the CORA toolbox to compute the PRS as a sequence of zonotopes
%         \3 introduce zonotopes
%         \3 The CORA toolbox needs three inputs to compute the PRS:
%             \4 An initial condition set defined as a zonotope
%             \4 A dynamic model (we use the planning model augmented with the trajectory parameters)
%             \4 A partition of the planning time horizon $T = [0,t\final]$
%         \3 One can show that the PRS zonotopes provably contain every trajectory of the planning model
% \end{outline}

\subsection{Error Reachable Set}\label{subsec:ERS}

We now compute the ERS to represent the upperbound on tracking error and the robot's forward occupancy in workspace.
% Recall that the PRS only contains plans; but, in Section \ref{sec:safe_RL}, we leverage the zonotope Minkowski sum to add the PRS and ERS together to represent plans \textit{including} tracking error and forward occupancy.
Computing the tracking error and forward occupancy requires performing reachability analysis on the high-fidelity model.
This is typically intractable with methods such as \cite{althoff2015cora} due to the high-dimensional, nonlinear nature of those models.
Instead, we use a sampling-based approach, find the forward occupancy error, and represent it as zonotope, and use that object to ensure safety.
We call such an object the Error Reachable Set.

To proceed, we do the following: (1) define tracking error, (2) explain how to partition $K$ and $X\hi$ to enable minimum over-approximation of the tracking error, (3) propose a new way to combine tracking error and robot occupancy into the ERS, (4) compute the ERS with Algorithm \ref{algo:ers}, and (5) explain how to choose samples such that our ERS representation is conservative.

\subsubsection{Tracking Error}
We define the \defemph{tracking error} as a trajectory $e: T \to \R^\plandim$, and
\begin{align}
    e(t;x\hiz,k) = p(t;x\hiz) - p\plan(t,k),\label{eq:tracking_error_defn}
\end{align}
\noindent where $p$ is the position subspace trajectory of
\begin{align}
    x\hi(t) = \int_0^t f\hi(x\hi(s),u\track(t,x\hi(s),k)ds + x\hiz,
\end{align}
and $x\hiz \in X\hi$ is such that $p(0) = 0$ and $\dot{p}\plan(0;k) = \dot{p}(0)$.
% \simon{why is $x\hiz$ not part of e, or it is implicitly?}
% \shrey{i guess we don't need proj or $\dot{P}$, but we need $f\ini: X\hi \to K$.
% Note to self, fix the $f\ini$ definition!}
Notice that, for any $u\track$ as in \eqref{eq:u_tracking_controller}, $e$ is bounded because $f\hi$ is Lipschitz and $T$, $U$, and $K$ are compact. 

% \shrey{
% Note to self, this following math helps me understand what the ERS is supposed to do.
% Our goal is to conservatively estimate a function
% \begin{align}
%     \reachset\err: T\times K \to \pow{\R^\workspacedim}
% \end{align}
% for which
% \begin{align}
%     \forwardoccupancy(x\hi(t)) \subset \reachset\err(t,k) \oplus \{p\plan(t,k)\},
% \end{align}
% where
% \begin{align}\begin{split}
%     &x\hi(t) = \int_0^t f\hi(x\hi(s),u\track(t,x\hi(s),k)ds + x\hiz,\\
%     &\proj_P(x\hiz) = 0,\ \regtext{and}\ x\hiz \in f\ini\inv(k).
% \end{split}\end{align}
% Note to self, this tells us how to define $f\ini$.
% }
% \simon{what is big E in 31?}
% \simon{notice if $\reachset\err$ can be over approximated, then we have what we need, therefore the goal is to find max tracking error for each t and k }
\subsubsection{Partitioning for Better Approximation} \label{sec:partition}
Recall we compute an upperbound on the tracking error to ensure safety of the robot. 
However, due to the mismatch between the non-linearity in the planning model and the high fidelity model, tracking error for different $k$ and $x\hiz$ can be vastly different.
Therefore, computing a single tracking error over-approximation for all plans from all initial conditions can be overly conservative.

\Ram{does this belong in an assumption box?} Now if we \textbf{assume} that plans(i.e. $k$) that are close to each other can be tracked by close high-fidelity initial conditions with similar tracking error, we can employ partitioning on parameter space $K$ and high fidelity initial condition space $X\hi$ to minimally over-approximate the tracking error in each partition.

The partitioning is done in the following way:
\begin{align}
    K &= \union_{j=1}^{m_{K}} K\idx{j}~\regtext{and}\\
    X\hi &= \union_{h=1}^{m_{X\hiz}} X\hi\idx{h}
\end{align}
\noindent such that each $K\idxj$ and $X\hi\idxh$ is an axis-aligned box, $K\idx{i}\cap K\idxj = \emptyset$ for any $i \neq j$, and $X\hi\idxi \cap X\hi\idxj = \emptyset$ for any $i \neq j$.
Based on the above assumption, at the cost of storage, a finer partitioning leads to less over-approximation of tracking error in each partition.

% We apply the algorithm proposed in \cite{bbox} to bound tracking error and finds minimum area rotated box as $(c,l,R)=\minbbfunc(V)$, where $V$ is a set of tracking error
% \shrey{Questions a confused reader will ask: what is a ``set'' of tracking error?
% Do you mean a set of tracking error trajectories?
% How do you generate such a set?}.
% We then represent the ERS by computing a zonotope $Z\err\idxfrs$ for each $T\idxi\times X\hi\idx{h}\times K\desi\idx{j}$ in our partition of $T\times X\hi\times K\desi$.
% \begin{align}
%   (c,l,R) = \minbbfunc( e(t;x\hiz,k)) \\
%   \forall t\in T\idxi,k\in K\idx{j}, x\hiz\in X\hi\idxh\\
%       Z\err\idx{i,j,h} \leftarrow \zono{c, R\,\diag{l}}.
% \end{align}
% These partitions allow us to create zonotopes that are less conservative than \eqref{eq:ers} but still over-approximating.


\subsubsection{Compensating for Forward Occupancy Error}
%  $\forwardoccupancy$ returns a rotated box containing the robot at the state $x\hi$.
% Then we don't need to talk about vertices or have any indices for the vertices.
% You can get the minBoundingBox of a collection of rotated boxes in the algorithm.

We improve the method on accounting for the forward occupancy of the robot by bounding the difference between forward occupancy map and the planning model, and calling that the FOError. 
We then bound the FOError for each partition of plans and high fidelity initial condition, and convert that into the ERS.
Prior work addressed this by adding volume to the ERS to contain every possible rotation of a robot \cite{kousik2019safe}.
This latter approach is conservative for an elongated robot body such as a car \cite[Sec. 4]{kousik2018bridging}.

We apply the algorithm $\minbbfunc$ proposed in \cite{bbox} to finds minimum area rotated box for the FOError of a partition of $K$ and $X\hi$, as
\begin{align}\label{eq:min_bbox_for_forward_occ}
    V &= \union_{(t,x\hiz,k) \in \mathcal{S}}\proj_P(\forwardoccupancy (x\hi(t;x\hiz,k)))  - p\plan(t,k) \\
    (c,l,R) &= \minbbfunc\left(V\right)\\
    Z\err\idx{i,j,h} &= \zono{c, R\,\diag{l}}.
\end{align}
where
\begin{align}\label{eq:sampleset_defn}
    \mathcal{S} = \{(t,x\hiz,k) \in T\idxi\times\samplefunc(X\hiz\idxh\times K\idxj)\}.
\end{align}
\shrey{Using $\proj_P$ on $\forwardoccupancy$ doesn't really make sense... what were you trying to say?}

\simon{$\samplefunc$ needs to be defined?}
\shrey{yep.
we can say it gets defined later on tho.}


\subsubsection{Computing the ERS via Sampling}


Consider a finite, discrete set $K\sample \subset K$ (we discuss how to choose $K\sample$ after presenting our algorithm to compute the ERS).
For each $k \in K\sample$, we can compute the tracking error as in \eqref{eq:tracking_error_defn} or \eqref{eq:vertex_tracking_error}.
Using Algorithm \ref{algo:ers}, we computes $Z\err$.
\shrey{need to fix the above sentences to make use of the partition of $K\times X\hi$ to match up with alg \ref{algo:ers}}
That is, we have obtained a zonotope representation of the ERS that is ready to be used online for safety check:
\begin{align}
    \ERS = \{Z\err\idxfrs\ |\ (i,j,h) \in \N_{n_T}\times\N_{m_K}\times \N_{m\hi}\}.
\end{align}


\begin{algorithm}[h] \label{algo:ers}
\caption{ERS Sampling}
\SetAlgoLined
requires $K,X\hi,T$ and how they are partitioned\\
\For{$(j,h) \in \N_{m_K}\times \N_{m_{x\hi}}$}{
    
    Create a set of a samples $\{k\idx{n},x\hiz\idx{n}\}_{n = 1}^{n_\regtext{samples}}\in K\idx{j}\times X\hi\idx{h}$\\
    \For{each sample $k\idx{n},x\hiz\idx{n}$}{
        Simulate trajectory and collect $\forwardoccupancy(x\hi(t;x\hiz\idx{n},k\idx{n}))- p\plan (t,k\idx{n})$ in FOError
       }
       
    \For{$i \in \N_{n_T}$}{
        $(c,l,R) = \minbbfunc(\regtext{FOError })\forall t \in T\idx{i}$
        
        $Z\err\idxfrs = \zono{c,R\diag{l}}$
        }
    }
\end{algorithm}

We make the following assumption to clarify the goal of our ERS computation algorithm.
\begin{assum}\label{ass:ERS_zonotopes_are_conservative}
Suppose $t \in T\idxi$, $k \in K\idxj$, and $x\hiz \in X\hiz\idxh$.
Suppose $Z\err\idxerr$ is computed using Algorithm \ref{algo:ers}.
We assume
\begin{align}
    \forwardoccupancy(x\hi(t;x\hiz,k)) \subset \{p\plan(t,k)\} \oplus Z\err\idxerr.
\end{align}
\end{assum}
\noindent In other words, the ERS zonotopes are conservative.
Next, we explain a sampling strategy for $\samplefunc$ to make it reasonable that this assumption is satisfied.
Note that it is reasonable to satisfy this assumption in practice, as validated empirically in both simulation and on hardware for a variety of robot morphologies \cite{kousik2018bridging,kousik2019safe,kousik2020_pcba,holmes2020reachable,shreyas_dissertation,vaskov2019not,vaskov2019towards}.
\shrey{need to fix citation style so these all lump together}
Finally, we note that, if one is unsure if Assumption \ref{ass:ERS_zonotopes_are_conservative} is satisfied, one can simply use larger $Z\err\idxerr$.

\subsubsection{Choosing Samples to Maximize Tracking Error}

We now present two propositions that explain our sampling strategy to generate a conservative ERS.
Then, we define $\samplefunc$.

Recall that the trajectory parameters are broken into $K\ini$ and $K\desi$.
\shrey{the previous subsection should just say, hey if we sample, we can compute an ERS.
then here, we say how to choose samples to be conservative (whereas random sampling might not be conservative)}
Our goal is to sample $k\ini$ and $k\desi$ to produce worst-case tracking error as in \shrey{ref the eq}.

We use the following to determine how to sample $k\ini$.
\begin{prop}\label{prop:tracking_error_max_at_max_k_init}
(\cite[Proposition 7.1]{shreyas_dissertation})
Consider a double integrator high-fidelity model with states $p$ and $\dot{p} \in \R$, control input $u \in \R$, and $\ddot{p} = u$.
Let $p\plan(\cdot,k): T \to \R$ be a smooth plan.
Suppose that
\begin{align}
    u = \gmp\cdot(p - p\plan) + \gmd\cdot(\dot{p} - \dot{p}\plan) + \ddot{p}\plan,
\end{align}
where $\gmp,\gmd \in \R$ are control gains and $\ddot{p}\plan$ is a feedforward term.
Suppose that $p(0,k) = p\plan(0,k) = 0$ and $\dot{p}(0,k) \in [\dot{p}\submin,\dot{p}\submax]$.
Then the tracking error magnitude $|p(t,k) - p\plan(t,k)|$ achieves a maximum over $t \in T$ and over all $\dot{p}(0,k)$ when $\dot{p}(0,k) \in \{\dot{p}\submin,\dot{p}\submax\}$.
\end{prop}
\noindent 
In other words, tracking error is maximized for a linear system tracking an arbitrary smooth plan when the initial velocity is either maximized or minimized.
Recall that the parameter subspace $K\ini$ determines the initial velocity of each plan.
So, if we assume that the robot's control inputs determine its acceleration, and that it uses a PD feedback controller, then we know that \textit{maximizing} the initial velocity magnitude maximizes tracking error for an arbitrary plan.


To sample $k\desi$, consider the following:
\shrey{note to self, make $\ddot{p}\plan(t,k) = f_1(k)f_2(t)$ where $f_2$ is a polynomial in $t$ and $f_1$ is monotonic in $k$, so that this proof is more generic}
\begin{prop}\label{prop:tracking_error_max_at_max_k_des}
Consider the model from Proposition \ref{prop:tracking_error_max_at_max_k_init}, and suppose $u$ has no feedforward term:
\begin{align}\label{eq:prop_k_desi_controller}
    u = \gmp\cdot(p - p\plan) + \gmd\cdot(\dot{p} - \dot{p}\plan).
\end{align}
Suppose $p(0) = p\plan(0,k)$.
Suppose $k = (k\ini,k\desi)$ with $k\ini$ fixed such that $\dot{p}(0,k) = \dot{p}\plan(0,k)$.
Consider a planning model $p\plan: T\times K \to \R$ for which, for all $t \in T$, $\ddot{p}\plan(t,k) = k\desi \in [k\submin,k\submax] \subset \R$ (that is, $K\desi$ is also 1-D).
Then the tracking error magnitude $|p(t) - p\plan(t)|$ is maximized when $k\desi \in \{k\submin,k\submax\}$.
\end{prop}
\begin{proof}
Consider the tracking error system
\begin{align}
    z(t,k) &= \begin{bmatrix}
            z_1(t,k) \\ z_2(t,k)
        \end{bmatrix} =
        \begin{bmatrix}
            p(t) - p\plan(t,k) \\ \dot{p}(t) - \dot{p}\plan(t,k)
        \end{bmatrix}.
\end{align}
Recalling that $\dot{k} = 0$ for any plan, we have
\begin{align}
    \dot{z}(t,k) &= \underset{A}{\underbrace{\begin{bmatrix}
            0 & 1 \\ \gmp & \gmd
        \end{bmatrix}}}z(t,k) +
        \begin{bmatrix}
            0 \\ \ddot{p}\plan(t,k)
        \end{bmatrix},\label{eq:prop_k_desi_proof_first_order_system}
\end{align}
for any fixed $k \in K$.
We can solve for $z$ to find
\begin{align}
    z(t,k) &= e^{At}z(0,k) + \int_0^t e^{A(t-s)}\begin{bmatrix}
            0 \\ \ddot{p}\plan(s,k)
        \end{bmatrix}ds\\
        &= 0 + \left(\int_0^t e^{A(t-s)}ds\right)\begin{bmatrix}
            0 \\ k\desi
        \end{bmatrix}\\
        &= -A\inv(e^{At} - I_{2\times 2})\begin{bmatrix}
            0 \\ k\desi
        \end{bmatrix},\label{eq:prop_k_desi_proof_particular_soln}
\end{align}
where $I_{2\times 2}$ is an identity matrix.
Notice that
\begin{align}
    A\inv = \begin{bmatrix}
            -\gmd/\gmp & 1/\gmp \\ 1 & 0
        \end{bmatrix},
\end{align}
and we can choose $\gmp$ and $\gmd$ such that
\begin{align}
    e^{At} = \begin{bmatrix}
            a_1(t) & a_2(t) \\ a_3(t) & a_4(t)
        \end{bmatrix}
\end{align}
with $a_2(t) \neq 0$.
Then, by expanding \eqref{eq:prop_k_desi_proof_particular_soln}, we have
\begin{align}
    z_1(t,k) = \frac{1 - a_2(t)}{\gmp} k\desi,
\end{align}
completing the proof.
\end{proof}
\noindent Note that the planning model in this proposition does not obey Definition \ref{def:plan} because $\dot{p}\plan(t\final,k)$ is not necessarily 0.
However, one can derive a similar result for a valid planning model with $\ddot{p}\plan(t,k) \propto (k\desi - k\ini)t^2$ as in Example \ref{ex:plan}.
\shrey{Note to self, might be worth just using a valid planning model in the proof to avoid confusing the reader.
If $\ddot{p}\plan(t,k) \propto (k\desi - k\ini)t^2$, we can apply integration by parts twice to the particular solution and get the same result with a bit more algebra.}

Notice that the proof assumes the control input is drawn from $U = \R$, but $U$ is defined to be compact for the high-fidelity model.
However, input saturation does not affect the result of Proposition \ref{prop:tracking_error_max_at_max_k_des}.
First, notice that if we include the feedforward term $\ddot{p}\plan$ in $u$ from \eqref{eq:prop_k_desi_controller}, then the tracking error is $0$ for all time without input saturation.
But, if the input is saturated, this is equivalent to a constant control input being applied in the solution to \eqref{eq:prop_k_desi_proof_first_order_system}, meaning that $\ddot{p}$ is a constant as in the proof.
Therefore, as we would expect, one can maximize tracking error by choosing $k\des$ to maximize input saturation (i.e., command the largest possible acceleration).

The takeaway message of Proposition \ref{prop:tracking_error_max_at_max_k_des} is that, for a system with acceleration as the control input, tracking error is maximized by choosing an extremum of $K\desi$.
Therefore, we should sample $k \in K$ that are extrema of $K\ini\times K\desi$.
Since $K$ is a finite-dimensional, compact box, it has a finite number of extrema (i.e., vertices), which means that using a sampling-based approach is reasonable for our application.
\shrey{I think we need to clarify why we want the worst-case tracking error}

\shrey{Note to self, say something about how this ERS proof is new but has been validated empirically on a variety of systems + hardware}

\shrey{Define $\samplefunc$ here using the vertices of $K\idxj$}


\begin{figure}[ht] \label{fig:err_bound}
\centering
\includegraphics[trim={3cm 0 6cm 0},clip,width=\linewidth]{Figure/ErrorBound.pdf}
\caption{To compute the maximum tracking error for the two sampled reference trajectories together at the sampled time instant below, we use the high fidelity model to track each reference trajectory(black) and plot the errors(yellow, cyan) with respect to the reference points(pink) for this sampled time instant in error coordinate. Then we bound the error using a minimum area rotated rectangle(red), and call that the max tracking error for the two sampled trajectories}
\label{fig:ERS}
\end{figure} 




==> Sections/Methods/Robot_Env_Model_old.tex <==
\section{Robot, Planning, and Environment}\label{sec:robot_and_env}

%\techtip{Every section should start with an intro paragraph explaining what the section is about.
% First summarize the section.
% Second, briefly describe the subsections in order, and explain briefly how they are related.
% Third, describe the main result of the section if there is, e.g., an important theorem, algorithm, etc.}

We now present how we model the robot, plan trajectories, and model the robot's surroundings.
First, we describe a robot's equations of motion with a \defemph{high-fidelity model}.
Second, since safe, real-time planning is typically challenging using such a model, we introduce a simplified \defemph{planning model}.
Third, we discuss the tracking controller the robot uses to track plans generated by the planning model.
Fourth, we define obstacles and safety.

\subsection{High Fidelity Model}\label{subsec:high-fid_model}

We express the robot's motion using a \defemph{high-fidelity model}, $f\hi: X\hi \times U \to \R^\hifiddim$, where we the robot's state space is $X\hi \subset \R^\hifiddim$ and its control input space $U \subset \R^\ctrldim$.
Then,
\begin{align}
    \dot{x}\hi(t) = f\hi(x\hi(t),u),
\end{align}
where $t \in T \subset \R$ is time, $x\hi: T \to \R^\hifiddim$ is a trajectory of the high-fidelity model, and $u \in U$ is the control input.
We require that $f\hi$ is Lipschitz continuous in $x\hi(t)$ and $u$, and that $T$, $X\hi$, and $U$ are compact, so that trajectories of the high-fidelity model exist.
% \techtip{Notice that the topic sentence of the above paragraph is kind of redundant WRT to the intro.
% This is because the reader may have skipped the previous paragraph, or the intro, or maybe just forgot what the high-fidelity model is.
% Your job is to guide the reader through potentially unfamiliar definitions and math \smiley}

Since we are only considering robots in simulation for now, we assume %the following:
% \begin{assum}
there is no modeling error between the high-fidelity model and the robot's equations of motion.
% \end{assum}
% \noindent
Note one can extend the proposed method to the case where a trajectory $x\hi$ only describes the robot motion to within an error bound \cite[Assum. 12 and Thm. 39]{kousik2018bridging}.
Since our goal is to represent robots moving through space, we introduce a special subspace of $X\hi$.
\begin{defn}\label{def:position_subspace}
    The robot's state $x\hi \in X\hi$ includes the robot's position $p$ in a \defemph{position subspace} $P \subset \R^\plandim$ ($\plandim = 2$ or $3$).
    % Furthermore, we require that the robot's generalized velocity $\dot{p}$ can be derived from states of  $x\hi$ that occupy a \defemph{velocity subspace} $\dot{P} \subset \R^\veldim$.
\end{defn}
\noindent The position subspace usually represents, e.g., the robot's center of mass or baselink position in a global coordinate frame.
% The velocity subspace may represent, e.g., linear and angular velocity of the robot as a function of speed and steering angle (see Ex. \ref{ex:hifid}).

We introduce the following operator to consider the robot's position or other coordinates on their own:
\begin{defn}\label{def:proj}
Let $X_i$ be a lower-dimensional subspace of $X\hi$.
The \defemph{projection operator}, $\proj_{X_i}: X\hi \to X_i$, projects points from $X\hi$ to $x\hi$ \Ram{typo?} via the identity relation \Ram{this is a confusing way to define a projection operator...}.
We often extend this operator to $\proj_{X_i}: \pow{X\hi} \to \pow{X_i}$ to project sets.
\end{defn}
\noindent So, a robot's position at $x\hi \in X\hi$ is $p = \proj_P(x\hi)$.
\shrey{do we ever project to spaces other than $P$?}\simon{when project to $K\desi$ during online}
\shrey{i can probably get rid of that, we'll see}


% %\myoutline{time discussion}
% Recall that in receding horizon planning, we plan for a finite time horizon into the future. 
% After executing for a short period of time, we replan based on the new state of the robot. 
% Since RTS+RL uses receding horizon planning as the backbone, we let time starts at 0 at the beginning of each planning iteration, without loss of generality (WLOG).
% We specify $t\final > 0$, $T=[0,\infty)$, where $t\final$ is the total time of each plan, for a trajectory that brakes to a stop. 

% We use two models in RTS for different purposes: A high fidelity model that is known and used as the ground truth for determining the future state of the robot; 
% A planning model which is used for generating reference trajectories in real time.
% Lastly, we define a Lower Level Controller(LLC) for the robot to track the trajectory generated by the planning model.

% The high fidelity model is used offline to generate the difference between robot state and the planning model. 
% It can be described by dynamics model $f\hi: X\hi\times U \rightarrow \R^n$ where $X\hi \subset \R\hifiddim$, and control input space as $U\subset \R\ctrldim$.
% \begin{align}
%     \dot{x}\hi(t) = f\hi(x\hi(t), u)
% \end{align}
% \begin{assum}
%     This high-fidelity model $f\hi$ perfectly describes the dynamics of the robot and is known. 
%     We can neglect the error introduced by solving differential equation for the future states using a sequence of $u$ numerically.
% \end{assum}
% \noindent This is a reasonable assumption since we are only considering robots in simulation.
% One can extend the proposed method to the case where $f\hi$ only describes the robot motion to within an error bound \cite[Assumption 12]{kousik2018bridging}.

% \simon{ are these below useful?}
% \shrey{this first one ensures the existence and uniqueness of high fid model trajectories, the second one was redundant}
% \begin{assum}\label{assum:compact_and_cont}
%     The spaces $X\hi$ and $U$ are compact, and the high-fidelity model is Lipschitz continuous in $x\hi$ and $u$
% \end{assum}

% %\myoutline{example high fid}
\Ram{this example comes out of the blue and its relevance is never described. In addition you have to describe why this model is reasonable by citing something.}
\newcommand{\lng}{_{\regtext{long}}}
\newcommand{\lat}{_{\regtext{lat}}}
\begin{ex}
\input{Sections/run_example/CarModel}
\end{ex}

%\myoutline{Planning Model}
\subsection{Planning Model}
% %\myoutline{receding-horizon discussion}
% \techtip{Here, i used a long topic sentence that justifies why we need a planning model, and reminds the reader that we're doing receding-horizon planning}
Our receding-horizon planning framework, necessitates fast, frequent replanning for real-time operation; doing so is typically challenging with a high-fidelity model directly, so we use a simpler planning model \Ram{and bound the error ... you should mention that here otherwise the reader may be primed to jump down our throats.}.

Before we define this model, we add structure to $T$.
Since the high-fidelity model is not time-varying, we denote $T = [0,t\final]$ (recall that we required it to be compact \Ram{but was it connected}).
That is, every plan begins at $t = 0$ without loss of generality (WLOG), and every plan is of duration $t\final$.

Now we define plans as follows:
\begin{defn}[Planning Model]\label{def:plan}
    Let $K \subset \R^\Kdim$ denote a compact space of \defemph{trajectory parameters}.
    The \defemph{planning model} is a map $p\plan: T\times K \to P$ that obeys three properties:
    \begin{enumerate}
        \item $p\plan$ is smooth almost everywhere $t \in T$ and $k \in K$,
        \item $p\plan(0,k) = 0$ for all $k \in K$, and
        \item $\dot{p}\plan(t\final,k) = 0$ for all $k \in K$.
    \end{enumerate}
    A single trajectory $p\plan(\cdot,k): T \to P$ is referred to as a \defemph{plan}.
\end{defn}
\noindent We use the smoothness of $p\plan$ to compute reachable sets in Section \ref{sec:offline_reachability}.
We fix $p\plan(0,k) = 0$ arbitrarily because we can transform (i.e., rotate and/or translate) any plan to the position/orientation of the high-fidelity model at the beginning of each planning iteration.
In other words, all plans are defined in the robot's local coordinate frame.
We fix $\dot{p}\plan(t\final,\cdot) = 0$ to ensure that all plans end with a stopping maneuver, which we call a \defemph{failsafe maneuver}.
This way, if the robot fails to find a safe plan in a planning iteration, it can continue executing a safe plan found in the previous iteration, enabling safety for all time \cite[Theorem 39]{kousik2018bridging}.
% \shrey{check the theorem number}
% \simon{this is the right thm}


% \techtip{Next, i introduce new vocabulary to the reader before using it}
% Consider a space $X \subset \R^\lofiddim$, which we specify as a subspace of $X\hi$ with $\lofiddim < \hifiddim$, so $\proj_X(X\hi) = X$.
% We also require that $P$ (Definition \ref{def:position_subspace}) is a subspace of $X$.
% Denote by $K \subset \R^\Kdim$ a compact space of \defemph{trajectory parameters} (discussed more below).
% We denote the planning model as $f: T\times K \to \R^\lofiddim$, for which
% \begin{align}
% \begin{split}\label{eq:planning_model}
%     \dot{x}(t;k) = f(t,k) \quad \regtext{and} \quad \dot{k}(t) = 0,
% \end{split}
% \end{align}
% where $x: T \to X$ is a \defemph{plan}, or trajectory of the planning model.
% The notation $x(t;k)$ indicates the plan is parameterized by $k \in K$. 
% We require $f$ to be Lipschitz in $t$ and $k$.
% We specify the initial condition for all plans as follows.
% Since the planning model $f$ is only dependent on time and parameters, the initial position of any plan can be arbitrary.
% Therefore, we require that all plans begin from a fixed position $p\ini \in P$.
% We can then transform (i.e., rotate and translate) a plan to the position of the high-fidelity model at the beginning of each planning iteration.

\subsubsection{Receding-horizon Timing}

We specify the rate at which the robot performs receding-horizon planning by defining a \defemph{planning time}, $t\plan \in (0,t\final)$.
In each planning iteration, if a new, safe plan is found before $t\plan$, the robot begins tracking it at time $t\plan$.
Otherwise, the robot continues executing the previous trajectory (which ends in a stop).
Therefore, ensuring the robot is safe for each plan generated by the planning model ensures it is persistently safe.

\begin{rem}
In each planning iteration, we predict where the robot will be at time $t\plan$ by forward-integrating the high-fidelity model for the duration $t\plan$ while it is tracking the previous plan; we discuss the feedback controller used for tracking plans below.
\end{rem}


\subsubsection{The Trajectory Parameter Space}\label{subsubsec:K_defn}

We require that the trajectory parameter space is an axis-aligned, box-shaped set.
\begin{defn}\label{def:K_param_space}
Let $\Kcenter, \Kdelta \in \R^\Kdim$.
Then
\begin{align}
    K = \boxset(\Kcenter,\Kdelta,0).
\end{align}
We also break the parameter space into two parts, so that $K = K\ini \times K\desi$.
Denote $k = (k\ini,k\desi) \in K$.
\end{defn}
% \noindent This definition is useful for computing reachable sets in Section \ref{sec:offline_reachability}.

The first part of $K$, $K\ini$, determines a plan's initial velocity, $\dot{p}\plan(0,k\ini)$; these parameters can be used to ensure that the plan begins at the same generalized velocity as the robot:
\begin{defn}\label{def:k_ini_convert_to_p_dot_ini}
\Ram{this looks like an assumption? Also does it really need to be surjective. Like suppose there was a $k\ini$ that did not correspond to $x\hi$ what would break? We just would never select/slice at that $k\ini$ at run-time?}
    We require the existence of a surjective \defemph{initial condition function}, $f\ini: X\hi \to K\ini$, for which $x\hi \mapsto k\ini$.
\end{defn}
\noindent Suppose the robot is at a state $x\hi$ and applying a control input $u$.
We implement $f\ini$ in general by setting the time derivatives of $p\plan(0,k) = \proj_P(f(x\hi,u))$ and solving for $k$.
\shrey{Note to self, may not need $\dot{P}$, and could just define $f\ini: K \to X\hi$ instead.
Then we can use $k\ini \in f\ini\inv(x\hiz)$ if needed for the ERS sampling alg.
I'll see what we need and come back to this}

\shrey{need to explain why $f\ini$ should be surjective}

The second part of $K$, $K\desi$ determines how the plan evolves during $t \in (0,t\final]$ (e.g., it specifies positions or velocities to be reached at particular times during a plan).
To perform planning, the RL agent chooses $k\desi$ in each receding-horizon planning iteration; that is, the RL network picks $k\desi$ instead of control inputs $u$.
Different choices of $k\desi$ may be safe or unsafe, whereas $k\ini$ is determined by the robot's state at $t = 0$.
This design choice of using $k\desi$ is an important feature of RTS+RL, because we can obtain stability guarantees and obey actuator limits using control techniques with respect to the parameterized trajectories, and then let RL focus on decision making.
One can also argue this is equivalent to using RL to pick segments of trajectories to solve a motion planning problem.

% The first part determines a desired state $x\desi(k\desi) \in X$ to be reached at time $t\peak$ (meaning, $x(t\peak;k) = x\desi(k\desi)$.
% Since RTS+RL uses receding horizon planning as the backbone, we let time starts at 0 at the beginning of each planning iteration, without loss of generality (WLOG).
% We specify $t\final > 0$, $T=[0,\infty)$, where $t\final$ is the total time of each plan, for a trajectory that brakes to a stop. 
% One important feature of RTS+RL is that the RL network proposes parameter $k\desi$ instead of control inputs $u$.
% This allows us to obtain stability guarantees and obey actuator limits using control techniques and focus RL on decision making.
% One can also argue this is using RL to pick segments of trajectories to solve a motion planning problem.
 
%  we specify the planning model with state space $X \subset \R\lofiddim$ as a time-varying dynamics $f: [0,t\final] \times K \to \R\lofiddim$ that depends on parameters $K\subset \R\Kdim$
% \begin{align}
%     \dot{x}(t;k) &= f(t,k)\\
%     \dot{k} &= 0
% \end{align}
% where $x: [0,t\final] \to X$ is a trajectory of the planning model and $x(t;k)$ indicates that the planned trajectory is parameterized by $k\in K$. 

% Each plan $x$ in each receding horizon planning iteration is split into two parts.
% In the first part $t\in [0,t\peak]$, the planning model should generate trajectory that leads the robot to a desired state specified by some parameters. 
% In the second part $t\in (t\peak, t\final]$, the planning model should generate a trajectory that bring the robot to a stop.
% We call the second part of each plan the failsafe trajectory. 
% As a result, if a new plan can be found in $t\peak$, the robot can start tracking a new reference trajectory starting from $t\peak$.
% Otherwise, the second part of the trajectory can be used to bring the robot to a stop.
% Therefore, ensuring the robot is safe for each plan generated by the planning model ensures it is always safe.



% The parameterization $K$ usually consists of two parts.
% The first part is related to the desired state $x\desi \in X$.
% We call those parameters $K\desi \in K$.
% The second part is related to the initial condition of the robot $x\ini\in X$.
% Those parameters are called $K\ini \in K$. 
% These parameters can be used to ensure the reference trajectory for the robot is smooth.

%\myoutline{car planning example}
To appreciate how this trajectory parameter space works, consider the following example:
\input{Sections/run_example/car_prs_ex}


\subsection{Tracking Controller}
To track a plan, we generate control inputs for the high-fidelity model using a \defemph{tracking controller}:
\begin{align}
    u\track: T\times X\hi\times K \to U.\label{eq:u_tracking_controller}
\end{align}
The controller applies control inputs to minimize the difference between the trajectory of high-fidelity model $x\hi$ and a planned trajectory $p\plan$. We call that difference \defemph{tracking error}.
Guaranteeing safety requires compensating for such tracking error; we present a method to do this in Sections \ref{sec:offline_reachability} and \ref{sec:safe_RL}.
One can construct a tracking controller for the vehicle model as follows:
\begin{ex}
\input{Sections/run_example/LLC}
\end{ex}

\subsection{Workspace and Forward Occupancy}
To maintain safe operation, we need the robot's whole body to avoid obstacles in the workspace.
Denote the workspace as $W \subset \R^\workspacedim$ ($\workspacedim \in {1,2,3}$).
Notice that the high-fidelity model and planning model typically only describe the motion the center of mass of a robot.
But, collision avoidance additionally requires reasoning about the robot's body.
Therefore we define the \defemph{forward occupancy map} $\forwardoccupancy: X\hi \to \pow{W}$, for which $\forwardoccupancy(x\hi) \subset W$ is the volume occupied by the robot at state $x\hi \in X\hi$.

We give an example of $\forwardoccupancy$ for the car below.
%, which relies on the following definition.
% \begin{defn} \label{def:box}
% We denote by $B(c, l, R)\subset \R^\arbdim$ a \defemph{rotated box}, defined by its center coordinate $c \in \R^\arbdim$ and its edges' lengths $l\in\R^\arbdim$, and its rotation $R\in \SO(\arbdim)$  with respect to a global coordinate frame:
% \begin{align}
%     B(c,l,r) = R\cdot\Big(&[-l\arridx{1},l\arridx{1}]\times[-l\arridx{2},l\arridx{2}]\times\cdots\\
%     &\cdots\times[-l\arridx{n},l\arridx{n}] + c\Big).
% \end{align}
% \end{defn}

\begin{ex}
The vehicle occupies a rectangular volume.
If $x\hi = (p,\psi,v,\delta)$ and $p = (p\lng,p\lat)$, then
\begin{align}
    \forwardoccupancy(x\hi) = \boxset\left(p,l,{\small\begin{bmatrix} \cos\psi & \sin\psi \\ -\sin\psi & \cos\psi\end{bmatrix}}\right)
\end{align}
where $l \in \R^2$ describes the lengths of the car's sides.
\end{ex}

\subsection{Environment Model}
Now we introduce the obstacles and environment assumptions to define safety. 
% with our safety  relation to them obstacles that appear in the environment the robot operates in.
A mobile robot often needs to operate in a environment with static or dynamic obstacles. 
Keeping a robot safe means that it must be collision-free with respect to surrounding obstacles.
For this work, we first assume the following for the obstacles.
\begin{assum}
    There are a finite number of obstacles. We assume each obstacle is $O = \boxset(c,l,R)\subset W$ , and static with respect to time. Moreover, there are in total $n$ obstacles, and we call the union of all obstacles
    \begin{align}
        X\obs =  \cup_{i\in n} O.
    \end{align}
\end{assum}
\noindent Note that this is a reasonable assumption because mapping and perception algorithms often output rotated boxes when building a map or recognizing obstacles \cite{yolov4,Thrun2003RoboticMA}.
We can extend this work to dynamics obstacles, as in \cite{vaskov2019towards,vaskov2019not} \Ram{probably want to say more here...}.


Now we define safety in the following way
\begin{defn}\label{def:obs}
If the forward occupancy map of the high fidelity model does not intersect with obstacles, i.e. 
\begin{align} \label{eq:safety_def}
    \forwardoccupancy(x\hi(t)) \cap X\obs = \emptyset,
\end{align}
then the robot is \defemph{safe}, otherwise we say that the robot is \defemph{in collision}.
\end{defn}

Since there is usually a limit on a robot's sensor radius.
For those situations, we assume that there is a max radius $d\sen$ called the \defemph{sensor horizon} 
\begin{assum}
    If the relative position of an obstacle to the robot position $\norm{x_{\regtext{obs}}-p}_2 < d\sen$, then it can be detected perfectly.
\end{assum}
\noindent where $ p \in P$ is the robot position, and $x\obs \in X\obs$ 
We have shown in previous work \cite{kousik2018bridging} that to ensure safety, we need $d\sen > v_{\regtext{max}}t\final+\Delta p\submax$, where $\Delta p\submax$ is the maximum distance that can be traveled by any planning trajectory, $v\submax$ the max velocity for the robot, which we assume in this work as well. \simon{@shreyas, take a look at section D}






==> Sections/PaperOutline.tex <==
\section*{Outline}
\begin{outline}
\1 \fig 1 as poster
\1 introduction
    \2 motivation
        \3 What problem is RL solving? Why useful?
        \4 RL tries to solve how software agents should take actions in an environment in order to maximize the long term cumulative reward. Useful since: general: they can handle nonlinear and stochastic(not using) dynamics and nonquadratic reward functions; evolving: improves based on the amount of data collected; fast, inference is fast(gradient descent is also fast as well since we have small network)
        \3 how do people try to enforce safety in RL? what are the challenges with RL?
        \4 Major weakness is RL doesn't do guarantees. Not safe for real world. People try to solve this using simplified(discrete) action space, rule based safety rules, reach-ability based safety layers. linear model approximation algorithm, etc
        
        \3 RTD is a way to enforce safety for motion planning, but does not incorporate learning -- what are the weaknesses of RTD? 
        \4 RTD is shortsighted, trajectory optimization step only considers the best local action to achieve a global goal.(Weakness of all Receding horizon planning) so may get stuck in local minimum. 
    
    \2 goal of this work: by combining RL + RTD, we can eliminate the disadvantages of both, and produce RTS for safe RL
    
    \2 contributions
        \3 algorithm for generating less conservative tracking error reachable sets for RTD
        \3 RTS: framework for leveraging RTD as a safety layer for RL
        \3 demonstration on three different robots
        
    \2 notation

\1 how we model the robot and its environment
    \2 time discussion
    \2 high-fidelity model describes the robot
        \3 \assume, since we're doing simulation, that this model is the actual robot.
        \3\assume compact and Lipschiz cont. \3\assume high fid exsists and bounded
        \3 \example car hi-fid model
    
    \2 planning model is simple enough to plan with in real time (because we can leverage the idea of parameterized trajectories)
        \3 important to point out how this is different from usual RL control input choice (do other methods also use parameterized trajectories?)\simon{ TUM one yes, they call it high level plans/lane change manuvers\cite{TUM_safe_lane_change_set_based}}
        \3 the planning model's dynamics are defined over a short time horizon, since this model is used for receding-horizon planning
        \3 to enable safety guarantees, we require every planning model to end with a fail-safe maneuver (in this work, that just means braking to a stop)
        \3 at runtime, the robot attempts to choose a new planning model trajectory at each receding-horizon planning iteration; since this is formulated as a nonlinear program for RTD\simon{not a program anymore, i guess just say adjust may take longer depending on how many paritions it visits.}, the robot is not typically guaranteed to find a new trajectory every $t\plan$ seconds, which is why every trajectory includes a braking maneuver
        \3 \example  car planning model \fig 2, top
    
    \2 tracking controller drives high-fidelity model towards planning model trajectories
        \3 \assume that the tracking error is bounded (this is reasonable since we can design a controller that only cares about the parameterized trajectories)
        \simon{is this one and the one in high-fid related}
        \shrey{i'm not sure what you mean, but i think yes they should be the same}
        
        \3 because the high-fidelity and planning models don't match up, we need to compensate for tracking error to say something about safety
        
        \3 \example car tracking, just two lines, maybe boring.
        
    \2 what does the environment look like?
        \3 obstacles are regions that the robot must not enter or else it has crashed (i.e., this is how we define safety) \simon{need to write}
        \3 \define obstacles are rotated box \simon{need to write}
            \4 also need to explain briefly why this is a reasonable definition
        \3 \define safety?
            \4 safety means that the robot's body does not intersect any obstacle
        \3 \assume obstacles are static
        \3 \assume the robot can sense all surrounding obstacles within a finite sensor horizon (cite \cite{kousik2018bridging}, no need to cover a ton of detail here)
        \3 point out that RTD extends to dynamic environments, so RTS can be extended to those as well \cite{vaskov2019towards,vaskov2019not}
        \3 \example sensor horizon and car obstacles \simon{need to write}
    
\1 enforcing safety using reachability analysis
    \2 we leverage the RTD framework
        \3 offline, RTD computes an FRS, which is a set containing trajectories of the high-fidelity model when tracking the parameterized trajectories with the feedback controller introduced earlier
        \3 online, RTD intersects the FRS with obstacles to identify which trajectories are unsafe
        
    \2 offline reachability analysis
        \3 \define the FRS (see \cite[(3.26)]{shreyas_dissertation}, in comparison with \cite[(6.20)]{shreyas_dissertation}, which defines a set of zonotopes \textit{containing} the FRS) \simon{need to write}
        \3 point out that we can think of it as a PRS + ERS 
            \4 \define PRS\simon{need to write}
            \4 \define ERS\simon{need to write}
        \3 zonotope representation allows us to create the PRS and ERS separately
            \4 \define zonotopes
            \4 \define minkowski sum of zonotopes
            \4 \define slice
        \3 numerical implementation of PRS
        \simon{you mean zonotope PRS, or CORA}
            \4 refer \fig 2, bottom
        \3 numerical implementation of ERS
            \4 talk about current version, algo 1
            \4 point out what's missing (i.e., state your contribution)
            \4 \example of tracking bounding error. \fig 3
    
    \2 online planning
        \3 explain what the constraints look like in terms of the FRS
        \3 numerical implementation of constraints (cite \cite{holmes2020reachable} and \cite{shreyas_dissertation} probably)
        \3 briefly explain RTD's trajectory optimization and point out what's missing \simon{need to write}
        
    
\1 safe reinforcement learning \simon{need to write}
    \2 offline training
        \3 for safe training, we use the FRS to make constraints, then adjust RL agent and penalize its reward based on how much it violated the constraints (right?, no, currently replacing distance not used, but to use it just 1 line change)
        \4 replace algorithm 
        \4 \example  replace \simon{need to write} refer \fig 1
        \3 for unsafe training, we just let the RL agent pick whichever parameters it wants (do you still give the agent a penalty, but just don't adjust its choice?)\simon{no penalty}
        
    
    \2 online testing
        \3 we can also use the FRS to enforce safety on the RL agent at runtime
        \3 if we don't enforce safety at runtime, the trained RL agent doesn't have any guarantees
        
\1 experiments
    \2\simon{I am doing it seperately for each robot}

    \2 robots, environments, and goals (refer to running example and appendices for more details)
        \3 cartpole on a finite-length track; goal is to achieve swingup without crashing
        \3 car on a highway with box-shaped obstacles; goal is to drive to end of road without crashing
        \3 quadrotor in a world with box-shaped obstacles; goal is to reach randomly-located goal without crashing
        \3 need to explain what the reward functions are (like minimize euclidean distance to the global goal)
        \3 need to point out that the robots and environments all obey the definitions in the section about how we model the robot and world        
        \3 make sure to point out what tracing controller each robot uses in the appendices
        
    \2 experimental design
        \3 offline training design (talk about comparison to safety on vs safety off)
        \3 online testing
            \4 I guess it's basically the same as training, but without doing training?
            \4 do you want to compare to vanilla RTD?
        
    \2 results
        \3 put results in tables
    
    \2 discussion (for each robot, do the following:)
        \3 why did/n't the results match your expectations?
        \3 if you noticed any unexpected behavior, what is a potential explanation?
        \3 what are the broader implications of the results (like, what general conclusions can you draw from the data?)
        
    \2 \shrey{I think it's worth seeing what happens when the RL agent is \textit{trained} with safety on but \textit{tested} with safety off}
    \simon{tried, for car, more success than safety on during evaluation, but more crashes as well. success/stopped/crashed: safety on: 91/9/0 safety off: 96/0/4}
    \shrey{perfect, that makes a lot of sense! super cool!}
\end{outline}


==> Sections/Related_work.tex <==

\begin{outline}

% \textbf{Ensuring safety with reachability}

\1 Reachibility is promising. There are some reach-ability based methods. However, these are either very conservative\cite{fisac2018general}, or very slow \cite{TUM_safe_lane_change_set_based}


\1 honorable mentions: 
\3 \cite{dalal2018safe} deals with continuous but assumes a linear model
\3 \cite{wabersich2018safe} Predictive filter

% \1 \chao{Is it supposed to be related work , not about our method? If you want to bring our method, we could bring this to the first sentence like our method is inspired by xxx methods, because the other method only have this section for themselves}
% Our method addresses all of these problems by precomputing the over-approximating Forward Reachable Set(FRS) of a continuum of parameterized robot trajectories and using these online to ensure safety of the robot. We can ensure robot is collision free in workspace in realtime.

\end{outline}
 

==> Sections/run_example/CarModel.tex <==
\label{ex:hifid}
We use the following high-fidelity model, adapted from \cite{rasekhipour2016potential} to represent a car driving on a multi-lane road.
The state space of the vehicle is $x\hi = [p\lng,p\lat,\psi,v,\delta] \in X\hi$, with dynamics
% The position is $[p\lng,p\lat]\trans \in P$.
% The car's dynamics $\dot{x}\hi$ are given by
\begin{align}\label{eq:car_high-fid_model}
\dot{x}\hi = \frac{d}{dt}\left[\begin{array}{c}
        p\lng \\
        p\lat \\
        \psi \\
        v \\
        \delta
    \end{array}\right] &=
    \left[\begin{array}{c}
        v \cos\psi - v\lat \cos \psi \\
        v \sin\psi + v\lat \cos \psi \\
        \omega \\
        c_1 v + c_2 u_{1} \\
        c_3\cdot\left(u_{2}-\delta\right)
    \end{array}\right], \\
\omega &= \frac{v \tan \delta}{c_4 + c_5 v^{2}},\ \regtext{and}\\
v\lat &= \omega\left(c_6 + c_7 v^{2}\right),
\end{align}
% \begin{align} % OLD VERSION
% \frac{d}{d t}\left[\begin{array}{c}
% p\lng \\
% p\lat \\
% \psi \\
% v \\
% \delta
% \end{array}\right] &=\left[\begin{array}{c}
% v \cos\psi - v\lat \cos \psi \\
% v \sin\psi + v\lat \cos \psi \\
% \omega \\
% \frac{-T_{c}}{m} v + T_{c} u_{1} \\
% c_{w a}\left(u_{2}-\delta\right)
% \end{array}\right] \\
% \omega &=\frac{v \tan \delta}{l+\frac{c_{u s}}{g} v^{2}} \\
% v\lat &=\omega\left(l_{r}-m v^{2} \frac{l_{r}}{C_{r} l}\right)
% \end{align}
where $p\lng$, $p\lat$, and $\psi$ are the longitudinal, lateral position, and heading in the global reference frame; $v$ is the longitudinal velocity in the robot's local (body-fixed) coordinate frame ($v\lat$ is its lateral velocity), and $\delta$ is its steering angle.
% Note that the generalized velocity is a function of $v$, $\psi$, and $\delta$.
The control inputs are $u = [u_1,u_2]\trans \in U$ are the acceleration command $u_1$ and steering torque $u_2$.
The values $c_1,\cdots,c_7 \in \R$ are constant model parameters.





% We generate the \textbf{reference signals} with parameterized time-varying polynomial \cite{mueller_drone_motion}, using parameters $[\kappa_{pk},\kappa_{y},\kappa_{v},\kappa_{h}]$.
% During run-time, the network selects desired velocity change $\Delta\kappa_{pk}$ and desired y position change $\kappa_{y}$.
% Furthermore, the initial velocity $\kappa_{v}$ and initial heading $\kappa_h$ are determined by the state of the vehicle, to ensure the generated reference trajectory is smooth.
% \shrey{it's odd to have the heading state be $\psi$ but the heading gain be $k_h$}
% For failsafe trajectory, we choose to break to a stop for velocity reference, similar to \cite{kousik2019safe}, and to hold the reference y position constant.\\
% Combining the features discussed, the reference signal for velocity $vx_{ref}$ is
% % x_ref
% \begin{align}
% vx_{ref}(t, \kappa)=\frac{c_{1}(t, \kappa)}{6} t^{3}+\frac{c_{2}(t, \kappa)}{2} t^{2}+\kappa_{v} \label{eq:vx_ref}
% \end{align}
% \begin{align}
% \left[\begin{array}{c}
% c_{1}(t, \kappa) \\
% c_{2}(t, \kappa)
% \end{array}\right]=\frac{1}{\left(c_{3}(t)\right)^{3}}\left[\begin{array}{cc}
% -12  \\
% 6 c_{3}(t)
% \end{array}\right]\left[\begin{array}{c}
% \Delta_{vx}(t, \kappa)
% \end{array}\right]
% \end{align}
% \begin{align}
% c_{3}(t)=\left\{\begin{array}{ll}
% t_{\mathrm{pk}} & t \in\left[0, t_{\mathrm{pk}}\right) \\
% t_{\mathrm{f}}-t_{\mathrm{pk}} & t \in\left[t_{\mathrm{pk}}, t_{\mathrm{f}}\right]
% \end{array}\right.
% \end{align}
% \begin{align}
% \Delta_{vx}(t, \kappa)=\left\{\begin{array}{ll}
% \kappa_{\mathrm{pk}}-\kappa_{v} & t \in\left[0, t_{\mathrm{pk}}\right) \\
% -\kappa_{\mathrm{pk}} & t \in\left[t_{\mathrm{pk}}, t_{\mathrm{f}}\right]
% \end{array}\right.
% \end{align}
%For $vx_{ref}$, the time to desired velocity $t_{pk} = 2 \mathrm{s}$, and the failsafe time is 4 seconds, summing to a total planning horizon of $t_{f} = 6 \mathrm{s}$. Whereas for $y_{ref}$ below, time to desired y position $t_{mid} = 4 \mathrm{s}$, and the reference is held constant as a failsafe maneuver until $t_f$. 
% \chao{(Should we explain those hypermeter choice?)}
% In this implementation, $t_{pk} = 2 \mathrm{s}$, $t_{mid} = 4 \mathrm{s}$ and $t_{f} = 6 \mathrm{s}$.
% \shrey{you should justify why you chose these numerical values (e.g., they are based on the stopping distance of the car from 30 m/s or something)}
% If a set of safe parameters is found after 2 seconds from the start of the current reference trajectory, the new trajectory is executed. Note that unlike parameter $\kappa_v$, the initial y position $y_0$ is an offset added to the reference, becuase the reference can be shifted in $x,y$ coordinates freely. The $y_{ref}$ is
% % y ref
% \begin{align}y_{ref}(t,\kappa)=\begin{array}{c}
% \frac{c_{4}(t, \kappa)}{120} t^{5}+\frac{c_{5}(t, \kappa)}{24} t^{4}+\frac{c_{6}(t, \kappa)}{6} t^{3}-\Delta_{vy}(\kappa) t + y_{0}\label{eq:y_ref}
% \end{array}
% \end{align}
% \begin{align}
% \left[\begin{array}{c}
% c_{4}(t, \kappa) \\
% c_{5}(t, \kappa) \\
% c_{6}(t, \kappa)
% \end{array}\right]=\frac{1}{{c_{3}(t)}^{5}}\left[\begin{array}{ccc}
% 720 & -360 c_{7}(t)  \\
% -360 c_{7}(t) & 168 {c_{7}(t)}^{2}  \\
% 60 {c_{7}(t)}^{2} & -24 {c_{7}(t)}^{3} 
% \end{array}\right]\left[\begin{array}{c}
% \Delta_{py}(\kappa) \\
% \Delta_{vy}(\kappa) 
% \end{array}\right]
% \end{align}
% \begin{align}
% c_{7}(t)=\left\{\begin{array}{ll}
% t_{\mathrm{mid}} & t \in\left[0, t_{\mathrm{mid}}\right) \\
% t_{\mathrm{f}}-t_{\mathrm{mid}} & t \in\left[t_{\mathrm{mid}}, t_{\mathrm{f}}\right]
% \end{array}\right. \\
% \Delta_{py}(\kappa) = \left\{ \begin{array}{ll} \kappa_y - \Delta_{vy}(\kappa) & t \in\left[0, t_{\mathrm{mid}}\right) \\
% 0 & t \in\left[t_{\mathrm{mid}}, t_{\mathrm{f}}\right]
% \end{array}\right. \\
% \Delta_{vy}(\kappa) = \left\{ \begin{array}{ll} -\kappa_v \sin(\kappa_h) & t \in\left[0, t_{\mathrm{mid}}\right) \\
% 0 & t \in\left[t_{\mathrm{mid}}, t_{\mathrm{f}}\right] \end{array}\right.
% \end{align}

% A sample trajectory is generated using the (\ref{eq:vx_ref}) and (\ref{eq:y_ref}) is shown in Figure. \ref{fig:Parameters}

% \begin{outline}
% \1 Dynamics and LLC of vehicle \simon{Done}
% \2 (Maybe put in appendix) Dynamics\simon{Done}
% \2 LLC \simon{Done}
% \2 Control Action limits\simon{not that important, skipped}
% \1 Parameters and ref trajectories definition, and network actions\simon{Done}
% \2 We leverage Muller's polynomial trajectory($\Delta v$ formulation for vx and $\Delta x$ formulation for y) as the trajectory generating model. A sample trajectory is shown in Figure. \ref{fig:Parameters} \simon{done}
% \2 The initial conditions are matched with the end state of the previous iteration so that the generated reference trajectory is always smooth. \simon{done}
% \2 A failsafe trajectory is always appended to the end of the desired trajectory, ensuring persistent feasibility\simon{done}
% \2 time split \simon{done}
 
% \end{outline}


%The first parameter stands for the desired peak velocity.
% the reference velocity reaches a peak at 2 seconds and decays down to 0m/s from 2 seconds to 6 seconds.
% The second parameter stands for the desired reference position change in the y direction. It gets gets to the desired y position at 4 seconds and remains constant from 4 seconds to 6 seconds.

% the main task of this paragraph is not about ho
% Section 4 explains how the Parameter generates the trajectories producing model of the ego car. This section describes how FRS could be obtained from this trajectories producing model

%param:k1 k2  ref traj Z(t):x,y,h,v,delta
%Tracking error is inevitable due to the controller and the environment condition. Under Figure xxx, red line represents the real value of the car, whereas the blue line is the theoretical value conducted based on Parameter(k1,k2) and time duration.The speed of the car and the trajectory of the car are highly dependent of parameter(k1,k2) and the time duration. In this example, k1 estimate the absolute velocity of the car after t1 second, and the velocity of the car will decay to zero if there is no further action needed. Similarly, k2 determines the relative trajectory change(in meter) after t2 second.

% /////K1 and K2 equations




%Refer to Figure \ref{fig:Parameters}, the car estimate speed change and the trajectory within the duration of 6 seconds. In this case, k1 is set to 5, and it indicates the car will reach a speed of 5m/s in 2 second and decays to 0 m/s if there is no further action needed. Similarly, k2 is set to -1 which indicates the car will shift 1 m to the right hand direction.


==> Sections/run_example/LLC.tex <==
% Here we present the low level controller (LLC) to control the car to its planning trajectory.
% Since the planning model state is a subspace of the high fidelity model space, we differentiate them by using $x\hi = [p\lng,p\lat,\psi,v\lng,\delta]$ for high fidelity states and $x = [r\lng, r\lat]$ for planning model states. 
% Here, $u_1, u_2$ are system inputs in Example \ref{ex:hifid}, and we have a specific plan $x$.
% \begin{align}
% u_{1}(t) &=k_{1}\left(v\des(t)-v\lng(t)\right) \\
% u_{2}(t) &=k_{2}\left(p\des(t)-y(t)\right)-k_{3} \psi(t)-k_{4} \delta(t)
% \end{align}
% where $k_1, k_2, k_3$ and $k_4$ are tuneable controller gains.
For the car from Example \ref{ex:hifid}, $P = P\lng\times P\lat$ and $x\hi = (p,\psi,v,\delta) \in \R^5$.
Let $p\plan$ be a plan with $k\ini$ determined by $x\hi$.
We specify $u\track$ as a PD controller:
% \begin{align}
%     u_k(t,x\hi(t),p(t,k)) =~&k_p(\proj_P(x\hi(t)) - p\plan(t,k)) + \\
%         &+k_v(v\lng(t) - \dot{p}\lng(t,k) + \\
%         &k_\psi(\psi(t) - 0) + k_\delta(\delta(t) - 0)
% \end{align}
\begin{align}
    u\track(t,x\hi(t)) = \Gamma\cdot\left(\begin{bmatrix} p(t) \\ \psi(t) \\ v(t) \\ \delta(t)  \end{bmatrix} -
    \begin{bmatrix} p\plan(t,k) + p_0 \\ 0 \\ v\plan(t,k) \\ 0 \end{bmatrix}\right),
\end{align}
where $\Gamma \in \R^{2\times 5}$ is a matrix of control gains, $p_0 = \proj_P(x\hi(0))$, and $v\plan(t,k) = \proj_{P\lng}(\dot{p}\plan(t,k))$.

==> Sections/run_example/car_prs_ex.tex <==
\begin{ex} \label{ex:plan}
For the car in Example \ref{ex:hifid}, we specify the planning model as piecewise polynomials adapted from \cite{mueller_drone_motion}.
Recall that $p = (p\lng, p\lat)$ for this model.
Let $K\ini, K\desi \subset \R^2$, and denote $k = (k\inione, k\initwo, k\desione, k\desitwo) \in K$.
The parameter $k\desione$ specifies a velocity to be reached at a time $t\desione \in (0,t\final)$, and $k\desitwo$ specifies a lateral position to be reached at a time $t\desitwo \in (0,t\final)$.
Denote $p\plan = (p_1, p_2)$.
The planning model is given by
\begin{align}
    p_1(t,k) &= \frac{\tau_1(t, k)}{24} t^{4} + \frac{\tau_2(t, k)}{6} t^{3} + k\inione t \label{eq:v_lng_ref}, \\
    p_2(t,k) &= \frac{\tau_4(t, k)}{120} t^{5} + \frac{\tau_5(t, k)}{24} t^{4} + 
        \frac{\tau_6(t, k)}{6} t^{3} - \Delta_{v\lat}(k) t,\label{eq:v_lat_ref}
\end{align}
where $\tau_1,\cdots,\tau_7$ are piecewise constant in $t$, with
\begin{align}
    \begin{bmatrix}
        \tau_1(t,k) \\ \tau_2(t,k)
    \end{bmatrix} &=
    \frac{\Delta_{v\lng}(t,k)}{\left(\tau_3(t)\right)^{3}}
    \begin{bmatrix}
        -12  \\ 6 \tau_3(t)
    \end{bmatrix},\\
    \tau_3(t) &= \begin{cases}
            t\desione & t \in [0,t\desione) \\
            t\final - t\desione & t \in [t\desione,t\final]
        \end{cases},\\
    \begin{bmatrix}
        \tau_4(t,k) \\ \tau_5(t, k) \\ \tau_6(t,k)
    \end{bmatrix} &= \frac{1}{{\tau_3(t)}^{5}} 
        \begin{bmatrix}720 & -360 \tau_7(t)  \\
            -360 \tau_7(t) & 168 {\tau_7(t)}^{2}  \\
            60 {\tau_7(t)}^{2} & -24 {\tau_7(t)}^{3} 
        \end{bmatrix}
        \begin{bmatrix}
            \Delta_{p\lat}(t,k) \\
            \Delta_{v\lat}(t,k) 
        \end{bmatrix},\\
    \tau_7(t) &= \begin{cases}
                t\desitwo & t\in [0,t\desitwo] \\
                t\final - t\desitwo & t\in [t\desitwo,t\final]
            \end{cases},\\
    \Delta_{v\lng}(t, k) &= \begin{cases}
            k\desione - k\inione & t \in [0, t\desione) \\
            -k\desione           & t \in [t\desione, t\final]
        \end{cases},\\
    \Delta_{p\lat}(t, k) &= \begin{cases}
            k\desitwo - \Delta_{v\lat}(t,k) & t \in [0, t\desitwo) \\
          0          & t \in [t\desitwo, t\final]
            \end{cases},\\
    \Delta_{v\lat}(t, k) &= \begin{cases}
            -k\inione\sin(k\initwo) & t \in [0, t\desitwo) \\
             0                      & t \in [t\desitwo, t\final]
            \end{cases}.
\end{align}
Example plans are shown in Figure \ref{fig:PRS}.
\end{ex}
\shrey{reminder to put implementation details in appendix}

\begin{figure}[ht]
\centering
\includegraphics[trim={1cm 0 1cm 0},clip,width=\linewidth]{Figure/RefvsZono.pdf}
\caption{The top subfigure shows plans as in Example \ref{ex:plan} at different $k\desitwo$ parameter values ranging from $[-1,1]$ m, with one specific trajectory shown in black.
The bottom subfigure shows the zonotope PRS for the same range of $k\desitwo$.
The black subset is the sliced PRS corresponding to the trajectory in the top subfigure.
\shrey{combine plans and zonotopes into a single plot, and remove the plot title}}
\label{fig:PRS}
\end{figure}

==> Sections/run_example/err_bound.tex <==
We partition the initial condition $\delta$ into 3 parts to limit conservatism.\simon{do i need more specifics here?}

To compute the tracking error, we use Algorithm \ref{algo:ers}. Figure. \ref{fig:err_bound} shows how to compute the error bound $e\idx{v}$ for one time instant $t$, one initial condition $x_{hi,0}$, two $\kappa_y$ values.
